Pairwise sequence alignment with block and character edit operations

Pairwise sequence comparison is one of the most fundamental problems in string processing. The most common metric to quantify the similarity between sequences S and T is edit distance, d(S,T), which corresponds to the number of characters that need to be substituted, deleted from, or inserted into S to generate T. However, fewer edit operations may be sufficient for some string pairs to transform one string to the other if larger rearrangements are permitted. Block edit distance refers to such changes in substring level (i.e., blocks) that "penalizes" entire block removals, insertions, copies, and reversals with the same cost as single-character edits (Lopresti & Tomkins, 1997). Most studies to calculate block edit distance to date aimed only to characterize the distance itself for applications in sequence nearest neighbor search without reporting the full alignment details. Although a few tools try to solve block edit distance for genomic sequences, such as GR-Aligner, they have limited functionality and are no longer maintained. Here, we present SABER, an algorithm to solve block edit distance that supports block deletions, block moves, and block reversals in addition to the classical single-character edit operations. Our algorithm runs in O(m^2.n.l_range) time for |S|=m, |T|=n and the permitted block size range of l_range; and can report all breakpoints for the block operations. We also provide an implementation of SABER currently optimized for genomic sequences (i.e., generated by the DNA alphabet), although the algorithm can theoretically be used for any alphabet. SABER is available at http://github.com/BilkentCompGen/saber

==> conclusion.tex <==
In this paper, we presented an algorithm, \algname, to address the block edit distance problem with traceback. Using simulations, we demonstrated its accuracy in detecting block edits between pairs of strings. However, since the general problem is known to be NP-Hard, an efficient optimal solution is evaded. Our algorithm would benefit all block edit distance computation applications, although the current implementation targets only genomic sequence rearrangements. We also note that, to our knowledge, although there is a wide range of theoretical work on this problem~\cite{Lopresti1997,Muthukrishnan2000,Cormode2002,Sahinalp2008}, \algname is the only block edit distance algorithm with an open source implementation.\footnote{We note that a similar tool, GR-Aligner, is no longer available for download on the web (URL \href{http://biocomp.iis.sinica.edu.tw/new/GR\_Aligner.htm}{http://biocomp.iis.sinica.edu.tw/new/GR\_Aligner.htm}).}

\algname supports several types of block edit operations together with the classical single-character edits; however, it currently does not detect \textit{block copies}. Our next aim will be to incorporate block copies into our formulation and implementation. Note that there exist algorithms for tandem block copies~\cite{Benson1997}; however, interspersed block copies should also be considered to cover the full picture of block edits. 
\algname currently has major drawbacks regarding run time and memory requirements, and it is not practically applicable for strings with $>$5,000 characters. Therefore, unlike marker-aware DCJ model-based tools~\cite{Bohnenkaemper2020}, it is not yet directly applicable to large problems, such as whole genome rearrangement discovery. However, it can still be used for refining the alignments of ``suspect'' regions that may harbor such rearrangements. Alternatively, it can be used as a secondary alignment step for read mapping tools (e.g., minimap2~\cite{Li2018}) for those DNA sequences reads that cannot be confidently aligned using the more widely used pairwise alignment algorithms~\cite{Alser2021} including the Smith-Waterman algorithm~\cite{Smith1981}. We leave these proposed enhancements and integrations as future work. We expect that along with further improvements in accuracy and speed, \algname will help better characterize genomic rearrangements together with other possible use cases of string comparisons.

